Multi-step Greedy Reinforcement Learning Algorithms

Multi-step greedy policies have been extensively used in model-based reinforcement learning (RL), both when a model of the environment is available (e.g.,~in the game of Go) and when it is learned. In this paper, we explore their benefits in model-free RL, when employed using multi-step dynamic programming algorithms: $\kappa$-Policy Iteration ($\kappa$-PI) and $\kappa$-Value Iteration ($\kappa$-VI). These methods iteratively compute the next policy ($\kappa$-PI) and value function ($\kappa$-VI) by solving a surrogate decision problem with a shaped reward and a smaller discount factor. We derive model-free RL algorithms based on $\kappa$-PI and $\kappa$-VI in which the surrogate problem can be solved by any discrete or continuous action RL method, such as DQN and TRPO. We identify the importance of a hyper-parameter that controls the extent to which the surrogate problem is solved and suggest a way to set this parameter. When evaluated on a range of Atari and MuJoCo benchmark tasks, our results indicate that for the right range of $\kappa$, our algorithms outperform DQN and TRPO. This shows that our multi-step greedy algorithms are general enough to be applied over any existing RL algorithm and can significantly improve its performance.

==> sections/GammaVariation.tex <==
\section{Comparison with Lowering the Discount Factor}

==> sections/rebuttal.tex <==
\clearpage

\section{Rebuttal Results}

\subsection{CartPole}
In this section, we analyze the role $\kappa$ plays in the proposed methods by reporting results on the simple CartPole environment for $\kappa$-PI TRPO. For all experiments, we use a single layered value function network and a linear policy network. Each hyperparameter configuration is run for 10 different random seeds and plots are shown for a 50\% confidence interval.

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.3]{Images/Rebuttal/CartPole_KPI_nkappa_x7.jpg}
    \includegraphics[scale=0.3]{Images/Rebuttal/CartPole_KPI_nkappa_1.jpg}
    \caption{Training performance of $\kappa$-PI-TRPO (Left) and the `naive' baseline $N(\kappa)=T$ (Right) on the CartPole environment.}
    \label{fig:CartPole}
\end{figure}

Note that since the CartPole is extremely simple, we do not see a clear difference between the $\kappa$ values that are closer to 1.0 (see Figure \ref{fig:CartPole}). Below, we observe the performance when the discount factor $\gamma$ is lowered (see Figure \ref{fig:CartPoleGamma}). Since, there is a ceiling of $R=200$ on the maximum achievable return, it makes intuitive sense that observing the $\kappa$ effect for a lower gamma value such as $\gamma=0.36$ will allow us to see a clearer trade-off between $\kappa$ values. To this end, we also plot the results for when the discount factor is set to 0.36.

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.3]{Images/Rebuttal/CartPole_gamma.jpg}
    \includegraphics[scale=0.3]{Images/Rebuttal/CartPole_KPI_nkappa_x7_gamma_036.jpg}
    \caption{Training performance when lowering the discount factor (Left) and of $\kappa$-PI-TRPO (Left) when discount factor is set to 0.36 (Right) on the CartPole environment.}
    \label{fig:CartPoleGamma}
\end{figure}

The intuitive idea behind $\kappa$-PI, and $\kappa$-VI similarly, is that at every time step, we wish to solve a simpler sub-problem, i.e. the $\gamma \kappa$ discounted MDP. Although, we are solving an easier/shorter horizon problem, in doing so, the bias induced is taken care of by the modified reward in this new MDP. Therefore, it becomes interesting to look at how $\kappa$ affects its two contributions, one being the discounting, the other being the weighting of the shaped reward (see eq. \ref{kappaContributionEquation}). Below we look at what happens when each of these terms are made $\kappa$ independent, one at a time, while varying $\kappa$ for the other term. To make this clear, we introduce different notations for both such $\kappa$ instances, one being $\kappa_{d}$ (responsible for discounting) and the other being $\kappa_{s}$ (responsible for shaping). 

\begin{equation}
\pi_\kappa(s) \in \arg\max_{\pi} \ \E[\sum_{t\geq 0} \underbrace{(\gamma\kappa_{d})^t}_{\text{discounting}} \lbrack r(s_t,a_t) + \underbrace{(1-\kappa_{s})\gamma V(s_{t+1})}_{\text{shaping}}] \mid s_0=s, \pi \rbrack, \quad \forall s\in\mathcal{S}
\label{kappaContributionEquation}
\end{equation}


\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.3]{Images/Rebuttal/CartPole_KPI_disc_nkappa_x7.jpg}
    \includegraphics[scale=0.3]{Images/Rebuttal/CartPole_KPI_shap_nkappa_x7.jpg}
    \caption{Training performance when contribution of $\kappa$ is fixed for a) the shaped reward (Left) and b) the discount factor (Right) on the CartPole environment.}
    \label{fig:kappaContribution}
\end{figure}

We see something interesting here. For the CartPole domain, the shaping term does not seem to have any effect on the performance (Figure \ref{fig:kappaContribution}(b)), while the discounting term does. This implies that the problem does not suffer from any bias issues. Thus, the correction provided by the shaped term is not needed. However, this is not true for other more complex problems. This is also why we see a similar result when lowering $\gamma$ in this case, but not for more complex problems.  

\subsection{Mountain Car}
In this section, we report results for the Mountain Car environment. Contrary to the CartPole results, where lowering the $\kappa$ values degraded the performance, we observe that performance deteriorates when $\kappa$ is increased. We also plot a bar graph, with the cumulative score on the y axis and different $\kappa$ values on the x axis.

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.3]{Images/Rebuttal/MountainCar_nkappa_x7.jpg}
    \includegraphics[scale=0.3]{Images/Rebuttal/MountainCar_KPI_nkappa_1.jpg}
    \caption{Training performance of $\kappa$-PI-TRPO (Top Left: training curves, Top Right: cumulative return) and the `naive' baseline $N(\kappa)=T$ (Bottom) on the Mountain Car environment.}
    \label{fig:MountainCar}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.3]{Images/Rebuttal/MountainCar_gamma.jpg}
    \includegraphics[scale=0.3]{Images/Rebuttal/MountainCar_KPI_nkappa_x7_gamma_0995.jpg}
    \caption{Training performance when lowering the discount factor (Left) and of $\kappa$-PI-TRPO (Left) when discount factor is set to 0.995 (Right) on the MountainCar environment.}
    \label{fig:MountainCarGamma}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.3]{Images/Rebuttal/MountainCar_KPI_disc_nkappa_x7.jpg}
    \includegraphics[scale=0.3]{Images/Rebuttal/MountainCar_KPI_shap_nkappa_x7.jpg}
    \caption{Training performance when contribution of $\kappa$ is fixed for a) the shaped reward (Left) and b) the discount factor (Right) on the MountainCar environment.}
    \label{fig:MountainCarkappaContribution}
\end{figure}

We use the continuous Mountain Car domain here, which has been shown to create exploration issues. Therefore, without receiving any positive reward, using a $\kappa$ value of 0 in the case of discounting (solving the 1 step problem has the least negative reward) and of 1 in the case of shaping results in the best performance. 

\subsection{Pendulum}

In this section, we move to the Pendulum environment, a domain where we see a non-trivial best $\kappa$ value. This is due to there not being a ceiling on the maximum possible return, which is the case in CartPole.

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.3]{Images/Rebuttal/Pendulum_KPI_nkappa_x7.jpg}
    \includegraphics[scale=0.3]{Images/Rebuttal/Pendulum_KPI_nkappa_1.jpg}
    \caption{Training performance of $\kappa$-PI-TRPO (Top Left: training curves, Top Right: cumulative return) and the `naive' baseline $N(\kappa)=T$ (Bottom) on the Pendulum environment.}
    \label{fig:Pendulum}
\end{figure}

Choosing the best $\gamma$ value and running $\kappa$-PI on it results in an improved performance for all $\kappa$ values (see Figure \ref{fig:PendulumGamma}). 

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.3]{Images/Rebuttal/Pendulum_KPI_gamma.jpg}
    \includegraphics[scale=0.3]{Images/Rebuttal/Pendulum_KPI_nkappa_x7_gamma_096.jpg}
    \caption{Training performance when lowering the discount factor (Left) and of $\kappa$-PI-TRPO (Left) when discount factor is set to 0.96 (Right) on the Pendulum environment.}
    \label{fig:PendulumGamma}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.3]{Images/Rebuttal/Pendulum_KPI_disc_nkappa_x7.jpg}
    \includegraphics[scale=0.3]{Images/Rebuttal/Pendulum_KPI_shap_nkappa_x7.jpg}
    \caption{Training performance when contribution of $\kappa$ is fixed for a) the shaped reward (Left) and b) the discount factor (Right) on the Pendulum environment.}
    \label{fig:PendulumkappaContribution}
\end{figure}

To summarize, we believe that in inherently short horizon domains (dense, per time step reward), such as the Mujoco continuous control tasks, the discounting produced by $\kappa$-PI and VI is shown to cause major improvement in performance over the TRPO baselines. This is reinforced by the results of lowering the discount factor experiments. On the other hand, in inherently long horizon domains (sparse, end of trajectory reward), such as in Atari, the shaping produced by $\kappa$-PI and VI is supposed to cause the major improvement over the DQN baselines. Again, this is supported by the fact that lowering the discount factor experiments actually result in deterioration in performance.  

\newpage
\subsection{Smoothness in $\kappa$}

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.23]{Images/Rebuttal/HalfCheetah_bar_KPI_nkappa_x7.jpg}
    \includegraphics[scale=0.23]{Images/Rebuttal/Ant_bar_KPI_nkappa_x7.jpg}
    \caption{Cumulative training performance of $\kappa$-PI-TRPO on HalfCheetah (Left, corresponds to Figure 12) and Ant (Right, corresponds to Figure 11) environments.}
    \label{fig:Smoothness}
\end{figure}


